Diverse by Design: Architectural Constraints for Prototype-Based Interpretability

Prototype-based neural networks provide inherent interpretability through case-based reasoning, yet suffer from critical limitations: prototypes converge to redundant features, fail to capture diverse semantic parts, and lack quantitative interpretability assessment. We propose Diversity-Aware Prototype Learning (DAPL), which enforces prototype diversity through architectural constraints rather than explicit regularization. Our approach leverages multi-head self-attention with strict one-to-one attention-to-prototype mapping, ensuring each prototype specializes in distinct visual features. We further introduce foreground-aware training to focus prototypes on semantically meaningful regions and develop comprehensive evaluation metrics (Coverage and Diversity) for quantitative interpretability assessment. Experiments on CUB-200-2011 demonstrate substantial improvements: DAPL with foreground-aware training achieves 81.69\% accuracy with 0.596 Coverage and 0.427 Diversity, providing the best overall balance across all evaluated prototype-based methods. Code is available at https://github.com/xinmiaolin/DAPL.

==> sec_4page/0_abstract.tex <==
% \begin{abstract}
% Prototype-based neural networks provide inherent interpretability through case-based reasoning, yet suffer from critical limitations: prototypes converge to redundant features, fail to capture diverse semantic parts, and lack quantitative interpretability assessment. We propose Diversity-Aware Prototype Learning (DAPL), which enforces prototype diversity through architectural constraints rather than explicit regularization. Our approach leverages multi-head self-attention with strict one-to-one attention-to-prototype mapping, ensuring each prototype specializes in distinct visual features. We further introduce foreground-aware training to focus prototypes on semantically meaningful regions and develop comprehensive evaluation metrics (Coverage and Diversity) for quantitative interpretability assessment. Experiments on CUB-200-2011 demonstrate substantial improvements: DAPL achieves 81.57\% accuracy with +5.44\% improvement and +32\% Coverage gain, while foreground-aware training further boosts performance to 82.02\% with superior interpretability.

% \end{abstract}

\begin{abstract}
Prototype-based neural networks provide inherent interpretability through case-based reasoning, yet suffer from critical limitations: prototypes converge to redundant features, fail to capture diverse semantic parts, and lack quantitative interpretability assessment. We propose Diversity-Aware Prototype Learning (DAPL), which enforces prototype diversity through architectural constraints rather than explicit regularization. Our approach leverages multi-head self-attention with strict one-to-one attention-to-prototype mapping, ensuring each prototype specializes in distinct visual features. We further introduce foreground-aware training to focus prototypes on semantically meaningful regions and develop comprehensive evaluation metrics (Coverage and Diversity) for quantitative interpretability assessment. Experiments on CUB-200-2011 demonstrate substantial improvements: DAPL with foreground-aware training achieves 81.69\% accuracy with 0.596 Coverage and 0.427 Diversity, providing the best overall balance across all evaluated prototype-based methods. Code is available at \url{https://github.com/xinmiaolin/DAPL}.


\end{abstract}


==> sec_4page/1_intro.tex <==
% \section{Introduction}
% \label{sec:intro}

% Deep learning has achieved remarkable success in computer vision, but its black-box nature limits deployment in high-stakes domains requiring transparency. Prototype-based neural networks~\cite{this-that,protopshare,pixel-grounded} offer an inherently interpretable alternative: they learn prototypical visual patterns and classify by measuring similarity to learned prototypes, providing case-based reasoning that mirrors human cognition.

% \begin{figure}[t]
% \centering
% \includegraphics[width=1.0\linewidth]{workshop_submission/images/dapl_intro-small.jpg}
% \caption{\textbf{Motivation: Prototype redundancy in existing methods.} ProtoPNet learns multiple redundant prototypes (left) focusing on similar wing regions, while DAPL (right) achieves diverse coverage of anatomical features.}
% \label{fig:motivation}
% \end{figure}

% Existing methods, however, suffer from prototype redundancy. Optimization dynamics favor learning multiple prototypes capturing similar discriminative features, because standard objectives lack explicit diversity mechanisms. As shown in Figure~\ref{fig:motivation}, ProtoPNet learns 6 of 10 prototypes on nearly identical wing patterns while missing other anatomical features. Moreover, prototypes often activate on background regions rather than meaningful object parts.

% We address these limitations with \emph{Diversity-Aware Prototype Learning (DAPL)}, which enforces prototype diversity via architectural constraints rather than explicit regularization. Our key insight is that multi-head self-attention naturally learns diverse spatial relationships—each head specializes in different visual patterns without explicit supervision. By enforcing strict one-to-one mapping between attention heads and prototypes, we architecturally guarantee this specialization transfers to the prototype level, preventing the redundancy that emerges from unconstrained optimization. We complement this structural constraint with contrastive regularization that explicitly maximizes inter-head prototype distinctiveness, ensuring each attention head learns truly unique visual patterns.

% Beyond the architecture, we introduce \emph{foreground-aware training} that penalizes prototype activations on background regions. While background context can provide useful cues for classification, over-reliance on background features reduces model transparency. Our foreground loss encourages the model to weight object-relevant features more heavily while still allowing contextual information to contribute.% when beneficial. 
% %For datasets without segmentation annotations, we substitute automatically generated segmentation methods. For example, in the domain of facial manipulation detection, we generate masks using facial landmarks combined with SAM~\cite{SAM} refinement. 

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.95\linewidth]{workshop_submission/images/DAPL_1to1.pdf}
% \caption{\textbf{DAPL Architecture.} (A) CNN backbone extracts features. (B) Multi-head self-attention produces $N$ diverse outputs. (C)~One-to-one mapping assigns each attention head to specific prototypes. (D) Similarity computation drives classification.}
% \label{fig:architecture}
% \end{figure*}

% To assess these ideas, we propose two new metrics: %systematically
% %leveraging ground-truth part annotations: 
% \emph{Coverage} and \emph{Diversity}. Coverage quantifies how well prototypes align with semantic object parts from ground-truth part annotations, measuring whether the learned representations capture meaningful visual concepts. Meanwhile, Diversity assesses whether prototypes are spatially distinct and evenly distributed across different parts.

% Our contributions are:
% \begin{itemize}
% \item A novel architecture combining multi-head self-attention with one-to-one attention-to-prototype mapping and contrastive regularization to enforce prototype diversity.
% \item Foreground-aware training that guides prototypes toward semantically meaningful object regions.
% \item Comprehensive evaluation metrics (Coverage and Diversity) for quantitative assessment of interpretability.
% \end{itemize}

% %DAPL achieves 81.57\% accuracy with +5.44\% improvement and +32\% Coverage gain, while foreground-aware training further boosts performance to 82.02\% with superior interpretability.
% Extensive experiments on CUB-200-2011 (with additional results on FaceForensics++ in the Appendix) demonstrate substantial improvements: DAPL alone achieves +5.44\% accuracy with 33\% Coverage gain over ProtoPNet, showing that architectural constraints effectively enforce diversity in learned representations. Foreground-aware training further adds 54\% Diversity over DAPL alone, and also greatly aids in visual interpretability.  

\section{Introduction}
\label{sec:intro}

Deep learning has achieved remarkable success in computer vision, but its black-box nature limits deployment in high-stakes domains requiring transparency. Prototype-based neural networks~\cite{this-that,protopshare,pixel-grounded} offer an inherently interpretable alternative: they learn prototypical visual patterns and classify by measuring similarity to learned prototypes, providing case-based reasoning that mirrors human cognition.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{workshop_submission/images/dapl_intro-small.jpg}
\caption{\textbf{Motivation: Prototype redundancy in existing methods.} ProtoPNet learns multiple redundant prototypes (left) focusing on similar wing regions, while DAPL (right) achieves diverse coverage of anatomical features.}
\label{fig:motivation}
\end{figure}

Existing methods, however, suffer from prototype redundancy. Optimization dynamics favor learning multiple prototypes capturing similar discriminative features, because standard objectives lack explicit diversity mechanisms. As shown in Figure~\ref{fig:motivation}, ProtoPNet learns 6 of 10 prototypes on nearly identical wing patterns while missing other anatomical features. Moreover, prototypes often activate on background regions rather than meaningful object parts.

We address these limitations with \emph{Diversity-Aware Prototype Learning (DAPL)}, which enforces prototype diversity via architectural constraints rather than explicit regularization. Our key insight is that multi-head self-attention naturally learns diverse spatial relationships---each head specializes in different visual patterns without explicit supervision. By enforcing strict one-to-one mapping between attention heads and prototypes, we architecturally guarantee this specialization transfers to the prototype level, preventing the redundancy that emerges from unconstrained optimization. We complement this structural constraint with contrastive regularization that explicitly maximizes inter-head prototype distinctiveness, ensuring each attention head learns truly unique visual patterns.

Beyond the architecture, we introduce \emph{foreground-aware training} that penalizes prototype activations on background regions. While background context can provide useful cues for classification, over-reliance on background features reduces model transparency. Our foreground loss encourages the model to weight object-relevant features more heavily while still allowing contextual information to contribute.% when beneficial. 
%For datasets without segmentation annotations, we substitute automatically generated segmentation methods. For example, in the domain of facial manipulation detection, we generate masks using facial landmarks combined with SAM~\cite{SAM} refinement.

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{workshop_submission/images/DAPL_1to1.pdf}
\caption{\textbf{DAPL Architecture.} (A) CNN backbone extracts features. (B) Multi-head self-attention produces $N$ diverse outputs. (C)~One-to-one mapping assigns each attention head to specific prototypes. (D) Similarity computation drives classification.}
\label{fig:architecture}
\end{figure*}

To assess these ideas, we propose two new metrics: %systematically
%leveraging ground-truth part annotations: 
\emph{Coverage} and \emph{Diversity}. Coverage quantifies how well prototypes align with semantic object parts from ground-truth part annotations, measuring whether the learned representations capture meaningful visual concepts. Meanwhile, Diversity assesses whether prototypes are spatially distinct and evenly distributed across different parts.

Our contributions are:
\begin{itemize}
\item A novel architecture combining multi-head self-attention with one-to-one attention-to-prototype mapping and contrastive regularization to enforce prototype diversity.
\item Foreground-aware training that guides prototypes toward semantically meaningful object regions.
\item Comprehensive evaluation metrics (Coverage and Diversity) for quantitative assessment of interpretability.
\end{itemize}

Extensive experiments on CUB-200-2011 (with additional results on FaceForensics++ in the Appendix) demonstrate substantial improvements: DAPL with foreground-aware training achieves 81.69\% accuracy with 0.596 Coverage and 0.427 Diversity, providing the best overall balance across all evaluated prototype-based methods.


==> sec_4page/2_related.tex <==
% \section{Related Work}

% \textbf{Prototype-Based Neural Networks.} ProtoPNet~\cite{this-that} pioneered case-based reasoning via similarity-based classification. Subsequent works explore cross-class sharing~\cite{protopshare}, pixel-level grounding~\cite{pixel-grounded}, deformable prototypes~\cite{deformable-protopnet}, differentiable assignment~\cite{protopool}, attention mechanisms~\cite{protoattend}, improved visualization~\cite{this-looks-like-those}, patch-based grounding~\cite{pip-net}, and domain-specific extensions~\cite{protomil,tesnet,st-protopnet,protoargnet,protosolo,protovae,lucidppn}. However, none explicitly address prototype redundancy or provide quantitative diversity metrics.

% \textbf{Attention Mechanisms for Interpretability.} Multi-head attention~\cite{attention_need,vit} naturally learns diverse feature representations. Recent advances include attention flow via Markov chains~\cite{attention-chains} and gradient-based ViT explainability~\cite{bousselham2025legrad}. Prototype-based ViTs~\cite{proto-vit,vit-net,protopformer,concepttransformer} show promise, but we focus on CNN backbones for compatibility with established baselines, leveraging attention to enforce diversity via one-to-one attention-to-prototype mapping.

% \textbf{Interpretability Evaluation.} Existing metrics address stability~\cite{con_stab_metrics}, consistency and purity~\cite{pip-net}, sparsity~\cite{protopnext}, and prototype quality~\cite{evaluation-protonet}, while broader approaches rely on human studies~\cite{mohseni2021multidisciplinary}, faithfulness scores~\cite{alvarez2018robustness}, deletion metrics~\cite{petsiuk2018rise,lin2021gradient}, or perturbation analysis~\cite{samek2017evaluating}. None directly assess prototype redundancy and semantic coverage. We introduce metrics for diversity and part alignment using ground-truth annotations.

\section{Related Work}

\textbf{Prototype-Based Neural Networks.} ProtoPNet~\cite{this-that} pioneered case-based reasoning via similarity-based classification. Subsequent works explore cross-class sharing~\cite{protopshare}, pixel-level grounding~\cite{pixel-grounded}, deformable prototypes~\cite{deformable-protopnet}, differentiable assignment~\cite{protopool}, attention mechanisms~\cite{protoattend}, improved visualization~\cite{this-looks-like-those}, patch-based grounding~\cite{pip-net}, and domain-specific extensions~\cite{protomil,tesnet,st-protopnet,protoargnet,protosolo,protovae,lucidppn}. However, none explicitly address prototype redundancy or provide quantitative diversity metrics.

\textbf{Attention Mechanisms for Interpretability.} Multi-head attention~\cite{attention_need,vit} naturally learns diverse feature representations. Recent advances include attention flow via Markov chains~\cite{attention-chains} and gradient-based ViT explainability~\cite{bousselham2025legrad}. Prototype-based ViTs~\cite{proto-vit,vit-net,protopformer,concepttransformer} show promise, but we focus on CNN backbones for compatibility with established baselines, leveraging attention to enforce diversity via one-to-one attention-to-prototype mapping.

% \textbf{Interpretability Evaluation.} Existing metrics address stability~\cite{con_stab_metrics}, consistency and purity~\cite{pip-net}, sparsity~\cite{protopnext}, and prototype quality~\cite{evaluation-protonet}, while broader approaches rely on human studies~\cite{mohseni2021multidisciplinary}, faithfulness scores~\cite{alvarez2018robustness}, deletion metrics~\cite{petsiuk2018rise,lin2021gradient}, or perturbation analysis~\cite{samek2017evaluating}. None directly assess prototype redundancy and semantic coverage. We introduce metrics for diversity and part alignment using ground-truth annotations.

\textbf{Interpretability Evaluation.} Existing metrics address stability~\cite{con_stab_metrics}, consistency and purity~\cite{pip-net}, sparsity~\cite{protopnext}, and prototype quality~\cite{evaluation-protonet}, while broader approaches rely on human studies~\cite{mohseni2021multidisciplinary}, faithfulness scores~\cite{alvarez2018robustness}, deletion metrics~\cite{petsiuk2018rise,lin2021gradient}, perturbation analysis~\cite{samek2017evaluating}, or transferable neural pathways~\cite{lin2023modelexplanationstransferableneural}. None directly assess prototype redundancy and semantic coverage. We introduce metrics for diversity and part alignment using ground-truth annotations.


==> sec_4page/3_methodology.tex <==

% %%%%%%%%% METHOD
% \section{Method}

% \subsection{Diversity-Aware Prototype Learning}

% Figure~\ref{fig:architecture} illustrates our approach. Given convolutional features $f(\mathbf{x}) \in \mathbb{R}^{H \times W \times D}$, we apply multi-head self-attention with $N$ heads to produce diverse spatial representations. Each attention head is assigned to specific prototypes through strict one-to-one correspondence, ensuring architectural diversity.

% Multi-head attention computes $Q = W_q f(\mathbf{x})$, $K = W_k f(\mathbf{x})$, $V = W_v f(\mathbf{x})$, then:
% \begin{equation}
% \mathbf{A} = \text{softmax}\left( \frac{Q K^T}{\sqrt{D_1}} \right) V \in \mathbb{R}^{N \times D_1 \times H \times W}
% \end{equation}
% where $D_1 = D/N$. Each $\mathbf{A}_h$ captures different spatial relationships.

% For one-to-one prototype assignment, each class $c \in \{1, ..., \mathcal{C}\}$ has $N$ prototypes, one per attention head. Attention head $h$ is exclusively compared with prototypes $\{\mathbf{p}_j | j = (k-1) \times N + h, k \in \{1, ..., \mathcal{C}\}\}$. For example, with $\mathcal{C}=200$ classes and $N=10$ heads, we have 2,000 prototypes: the first 10 belong to class 1 and pair with heads 1--10 respectively, the next 10 belong to class 2, and so on. Similarity is computed via:
% \begin{equation}
% s_{h,j}(\mathbf{x}) = \max_{h,w} \log \left( \frac{\|\mathbf{z}_{h,w} - \mathbf{p}_j\|_2^2 + 1}{\|\mathbf{z}_{h,w} - \mathbf{p}_j\|_2^2 + \epsilon} \right)
% \end{equation}

% We add contrastive regularization to explicitly enforce distinctiveness:
% \begin{equation}
% \mathcal{L}_{\text{contrast}} = \sum_{h=1}^N \sum_{\mathbf{p}_i \in \mathbf{P}_h} \sum_{\mathbf{p}_k \in \mathbf{P}_{\bar{h}}} \max(0, m - s_{h,i} + s_{h,k})
% \end{equation}
% where $m$ is a margin encouraging separation between assigned and unassigned prototypes.

% The similarity scores produce class logits through a fully-connected layer:
% \begin{equation}
% \text{logit}_c(\mathbf{x}) = \sum_{h=1}^N w_{c,h} \cdot s_{h,j_c^h}(\mathbf{x})
% \end{equation}
% where $w_{c,h}$ are learnable weights and $j_c^h$ denotes the prototype index for class $c$ and head $h$. Each classification decision thus aggregates evidence from diverse attention heads.

% \subsection{Foreground-Aware Training}

% To prevent background activation, we introduce foreground-aware training. Given foreground mask $\mathbf{m} \in \{0,1\}^{H \times W}$, we define background bias:
% \begin{equation}
% B(\mathbf{p}_j, \mathbf{x}, \mathbf{m}) = \frac{\sum_{h,w} (1-\mathbf{m}[h,w]) \cdot \mathbf{a}_{h,j}[h,w]}{\sum_{h,w} \mathbf{a}_{h,j}[h,w]}
% \end{equation}

% The foreground loss penalizes excessive background activation:
% \begin{equation}
% \mathcal{L}_{\text{fg}} = \frac{1}{|\mathcal{D}|} \sum_{\mathbf{x} \in \mathcal{D}} \frac{1}{m} \sum_{j=1}^m \max \left(0, B(\mathbf{p}_j, \mathbf{x}, \mathbf{m}) - \tau_{\text{bg}} \right)
% \end{equation}

% Total loss: $\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{ProtoPNet}} + \lambda_{\text{contrast}} \mathcal{L}_{\text{contrast}} + \lambda_{\text{fg}} \mathcal{L}_{\text{fg}}$, where $\mathcal{L}_{\text{ProtoPNet}}$ is the standard ProtoPNet objective combining classification, cluster, and separation losses~\cite{this-that}.

% \subsection{Evaluation Metrics}

% We propose Coverage and Diversity metrics using ground-truth part annotations. We first compute an overlap score between each prototype's activation region $A_j$ and part mask $M_k$: $\text{overlap}(\mathbf{p}_j, \text{part}_k) = |A_j \cap M_k|/|M_k|$, normalized by part size to ensure small parts (e.g., beak) are not underweighted. A prototype is assigned to a part when overlap exceeds threshold $\tau$.

% \textbf{Coverage} measures whether prototypes capture semantically meaningful parts via precision (fraction of prototypes assigned to $\geq 1$ part) and recall (fraction of parts captured by $\geq 1$ prototype):
% \begin{equation}
% \text{Coverage} = \frac{2 \cdot \text{Precision} \cdot \text{Recall}}{\text{Precision} + \text{Recall}}
% \end{equation}
% High Coverage indicates that prototypes align with most of the meaningful semantic features rather than missing features or capturing background information.

% \textbf{Diversity} combines two components: Redundancy, which quantifies spatial overlap (IoU) between prototypes assigned to the same part, and Imbalance, which measures uneven distribution of prototypes across parts using the Gini coefficient:
% \begin{equation}
% \text{Diversity} = 1 - \frac{\text{Redundancy} + \text{Imbalance}}{2}
% \end{equation}
% High Diversity indicates that prototypes are spatially distinct with balanced part coverage, rather than multiple prototypes redundantly focusing on the same features.



%%%%%%%%% METHOD
\section{Method}

\subsection{Diversity-Aware Prototype Learning}

Figure~\ref{fig:architecture} illustrates our approach. Given convolutional features $f(\mathbf{x}) \in \mathbb{R}^{H \times W \times D}$, we apply multi-head self-attention with $N$ heads to produce diverse spatial representations. Each attention head is assigned to specific prototypes through strict one-to-one correspondence, ensuring architectural diversity.

Multi-head attention computes $Q = W_q f(\mathbf{x})$, $K = W_k f(\mathbf{x})$, $V = W_v f(\mathbf{x})$, then:
\begin{equation}
\mathbf{A} = \text{softmax}\left( \frac{Q K^T}{\sqrt{D_1}} \right) V \in \mathbb{R}^{N \times D_1 \times H \times W}
\end{equation}
where $D_1 = D/N$. Each $\mathbf{A}_h$ captures different spatial relationships.

For one-to-one prototype assignment, each class $c \in \{1, ..., \mathcal{C}\}$ has $N$ prototypes, one per attention head. Attention head $h$ is exclusively compared with prototypes $\{\mathbf{p}_j | j = (k-1) \times N + h, k \in \{1, ..., \mathcal{C}\}\}$. For example, with $\mathcal{C}=200$ classes and $N=10$ heads, we have 2,000 prototypes: the first 10 belong to class 1 and pair with heads 1--10 respectively, the next 10 belong to class 2, and so on. Similarity is computed via:
\begin{equation}
s_{h,j}(\mathbf{x}) = \max_{h,w} \log \left( \frac{\|\mathbf{z}_{h,w} - \mathbf{p}_j\|_2^2 + 1}{\|\mathbf{z}_{h,w} - \mathbf{p}_j\|_2^2 + \epsilon} \right)
\end{equation}

We add contrastive regularization to explicitly enforce distinctiveness:
\begin{equation}
\mathcal{L}_{\text{contrast}} = \sum_{h=1}^N \sum_{\mathbf{p}_i \in \mathbf{P}_h} \sum_{\mathbf{p}_k \in \mathbf{P}_{\bar{h}}} \max(0, m - s_{h,i} + s_{h,k})
\end{equation}
where $m$ is a margin encouraging separation between assigned and unassigned prototypes.

The similarity scores produce class logits through a fully-connected layer:
\begin{equation}
\text{logit}_c(\mathbf{x}) = \sum_{h=1}^N w_{c,h} \cdot s_{h,j_c^h}(\mathbf{x})
\end{equation}
where $w_{c,h}$ are learnable weights and $j_c^h$ denotes the prototype index for class $c$ and head $h$. Each classification decision thus aggregates evidence from diverse attention heads.

\subsection{Foreground-Aware Training}

To prevent background activation, we introduce foreground-aware training. Given foreground mask $\mathbf{m} \in \{0,1\}^{H \times W}$, we define background bias:
\begin{equation}
B(\mathbf{p}_j, \mathbf{x}, \mathbf{m}) = \frac{\sum_{h,w} (1-\mathbf{m}[h,w]) \cdot \mathbf{a}_{h,j}[h,w]}{\sum_{h,w} \mathbf{a}_{h,j}[h,w]}
\end{equation}

The foreground loss penalizes excessive background activation:
\begin{equation}
\mathcal{L}_{\text{fg}} = \frac{1}{|\mathcal{D}|} \sum_{\mathbf{x} \in \mathcal{D}} \frac{1}{m} \sum_{j=1}^m \max \left(0, B(\mathbf{p}_j, \mathbf{x}, \mathbf{m}) - \tau_{\text{bg}} \right)
\end{equation}

Total loss: $\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{ProtoPNet}} + \lambda_{\text{contrast}} \mathcal{L}_{\text{contrast}} + \lambda_{\text{fg}} \mathcal{L}_{\text{fg}}$, where $\mathcal{L}_{\text{ProtoPNet}}$ is the standard ProtoPNet objective combining classification, cluster, and separation losses~\cite{this-that}.

\subsection{Evaluation Metrics}

We propose Coverage and Diversity metrics using ground-truth part annotations. We first compute an overlap score between each prototype's activation region $A_j$ and part mask $M_k$: $\text{overlap}(\mathbf{p}_j, \text{part}_k) = |A_j \cap M_k|/|M_k|$, normalized by part size to ensure small parts (e.g., beak) are not underweighted. A prototype is assigned to a part when overlap exceeds threshold $\tau$.

\textbf{Coverage} measures whether prototypes capture semantically meaningful parts via precision (fraction of prototypes assigned to $\geq 1$ part) and recall (fraction of parts captured by $\geq 1$ prototype):
\begin{equation}
\text{Coverage} = \frac{2 \cdot \text{Precision} \cdot \text{Recall}}{\text{Precision} + \text{Recall}}
\end{equation}
High Coverage indicates that prototypes align with most of the meaningful semantic features rather than missing features or capturing background information.

\textbf{Diversity} combines two components: Redundancy, which quantifies spatial overlap (IoU) between prototypes assigned to the same part—note that same-part assignment does not imply redundancy, as two ``wing'' prototypes may capture distinct subregions (e.g., wing tip vs.\ wing bar), and high IoU indicates they activate on the same pixels rather than complementary features—and Imbalance, which measures uneven distribution of prototypes across parts using the Gini coefficient. Imbalance captures the more critical failure mode where most prototypes concentrate on a few parts while others remain uncovered:
\begin{equation}
\text{Diversity} = 1 - \frac{\text{Redundancy} + \text{Imbalance}}{2}
\end{equation}
High Diversity indicates that prototypes are spatially distinct with balanced part coverage, rather than multiple prototypes redundantly focusing on the same features.


==> sec_4page/4_experiments.tex <==
% \section{Experiments}

% \subsection{Experimental Setup}

% \textbf{Dataset:} We evaluate on CUB-200-2011~\cite{cub-200} (11,788 bird images, 200 species, 15 part annotations). We use DenseNet-161 backbone with 2,000 prototypes (10/class), $N=10$ attention heads, and feature dimension $D_1=16$. Assignment threshold $\tau=0.2$.

% \textbf{Baselines:} ProtoPNet~\cite{this-that}, ProtoPShare~\cite{protopshare}, and PixPNet~\cite{pixel-grounded}.

% \subsection{Main Results}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_contrastive.pdf}\hfill
% \includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_foreground_coef.pdf}\hfill
% \includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_foreground_thresh.pdf}
% \caption{\textbf{Ablation studies on CUB-200-2011.} (Left) Contrastive loss coefficient $\lambda_c$: $\lambda_c=0.5$ achieves optimal Coverage. (Middle) Foreground loss coefficient $\lambda_{fg}$ (at $\tau_{bg}=0.3$): accuracy peaks at $\lambda_{fg}=15.0$. (Right) Foreground threshold $\tau_{bg}$ (at $\lambda_{fg}=20$): stricter thresholds improve both accuracy and Coverage.}
% \label{fig:ablation_studies}
% \end{figure*}

% \begin{table}[t]
% \centering
% \caption{Performance on CUB-200-2011 (DenseNet161).}
% \label{tab:main_cub}
% \begin{tabular}{lccc}
% \toprule
% \textbf{Method} & \textbf{Accuracy} & \textbf{Coverage} & \textbf{Diversity} \\
% & (\%) & $\uparrow$ & $\uparrow$ \\
% \midrule
% ProtoPNet & 76.13 & 0.443 & 0.152 \\
% ProtoPShare & 74.40 & 0.594 & 0.184 \\
% PixPNet & 76.68 & 0.250 & \textbf{0.450} \\
% \midrule
% DAPL ($D_1$=32) & 80.96 & 0.514 & 0.221 \\
% DAPL ($D_1$=16) & 81.57 & 0.589 & 0.277 \\
% DAPL ($D_1$=8) & 80.20 & 0.580 & 0.302 \\
% \midrule
% DAPL ($D_1$=16) + FG & \textbf{81.69} & \textbf{0.596} & 0.427 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth, trim={5.5cm 5cm 14cm 6cm}, clip]{workshop_submission/images/cub_head_dim_16.pdf}
% \caption{\textbf{Prototype activation comparison.} ProtoPNet (left) shows severe redundancy with 5 background and 2 wing prototypes. DAPL (right) achieves diverse coverage across 10 distinct anatomical parts. Class: American Goldfinch.}
% \label{fig:cub_comparison}
% \end{figure}

% Table~\ref{tab:main_cub} shows DAPL achieves \textbf{81.57\% accuracy} (+5.44\% over ProtoPNet) with \textbf{+33\% Coverage improvement} (0.443 $\rightarrow$ 0.589). Foreground-aware training further boosts accuracy to 81.69\% and Coverage to 0.596. While PixPNet achieves highest Diversity (0.450) through pixel-level grounding, it suffers from poor Coverage (0.250). ProtoPShare achieves better Coverage (0.594) but reduced accuracy (74.40\%). DAPL balances all metrics effectively. The optimal $D_1=16$ balances fine-grained details with sufficient context; smaller dimensions ($D_1=8$) enforce Diversity but lose accuracy, while larger ones ($D_1=32$) reduce Diversity and Coverage.

% Figure~\ref{fig:cub_comparison} illustrates the improvement: ProtoPNet exhibits severe redundancy with 5 background prototypes and 3 on identical wing patterns, missing critical features. DAPL achieves balanced coverage across 10 distinct anatomical regions (wing, back, belly, leg, crown, beak, neck, nape, forehead). This diversity stems from multi-head attention providing a natural architectural inductive bias—each head specializes in different spatial relationships—while our one-to-one mapping enforces this at the prototype level. Contrastive regularization further pushes prototypes toward distinct representations.

% Figure~\ref{fig:foreground_global} shows the effect of foreground-aware training: standard DAPL activations extend diffusely into the background, while foreground training localizes them tightly on specific bird parts, explaining the Coverage improvements in Table~\ref{tab:main_cub}.

% \subsection{Ablation Studies}

% We analyze key hyperparameters on CUB-200-2011 (Figure~\ref{fig:ablation_studies}). Contrastive coefficient $\lambda_c=0.5$ achieves optimal Coverage (0.600) and accuracy (80.98\%). Lower values ($\lambda_c=0.01$) provide insufficient diversity (Coverage 0.523), while excessive values ($\lambda_c \geq 1.0$) over-constrain the model (Coverage 0.434-0.579), suggesting that the architectural constraint alone is insufficient but must be complemented with moderate—not excessive—explicit regularization.

% \begin{figure}[t]
% \centering
% \includegraphics[width=1.0\linewidth, trim={1.6cm 2cm 1.6cm 4.2cm}, clip]{workshop_submission/images/foreground_comparison.pdf}
% \caption{\textbf{Foreground-aware training effect.} \textit{Top:} DAPL prototypes exhibit background bias. \textit{Bottom:} DAPL + FG focuses on meaningful bird parts.}
% \label{fig:foreground_global}
% \end{figure}

% Foreground coefficient $\lambda_{fg}$ shows accuracy improving from 81.17\% to 81.95\% at $\lambda_{fg}=15.0$, with Coverage peaking at 0.596 ($\lambda_{fg}=10.0$). This confirms that foreground guidance helps the model focus on discriminative object features rather than background context, improving both accuracy and interpretability simultaneously.

% Background threshold $\tau_{bg}$ analysis reveals that allowing minimal background activation ($\tau_{bg}=0.20$-$0.25$) is beneficial: accuracy improves from 80.79\% to 82.02\% and Coverage from 0.552 to 0.584. This suggests prototypes benefit from some boundary context, while overly strict thresholds ($\tau_{bg} < 0.10$) may exclude valid features at object edges.

% %%%%%%%%% CONCLUSION
% \section{Conclusion}

% We presented DAPL, addressing prototype redundancy through architectural constraints enforcing diversity. By leveraging multi-head self-attention with one-to-one prototype assignment and foreground-aware training, DAPL achieves +5.44\% accuracy improvement with +32\% Coverage gain on CUB-200-2011. Our evaluation framework provides quantitative metrics for systematic interpretability assessment, demonstrating that architectural inductive biases effectively enforce diversity in learned representations.

\section{Experiments}

\subsection{Experimental Setup}

\textbf{Dataset:} We evaluate on CUB-200-2011~\cite{cub-200} (11,788 bird images, 200 species, 15 part annotations). We use DenseNet-161 backbone with 2,000 prototypes (10/class), $N=10$ attention heads, and feature dimension $D_1=16$. Assignment threshold $\tau=0.2$.

\textbf{Baselines:} ProtoPNet~\cite{this-that}, ProtoPShare~\cite{protopshare}, and PixPNet~\cite{pixel-grounded}.

\subsection{Main Results}

\begin{figure*}[t]
\centering
\includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_contrastive.pdf}\hfill
\includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_foreground_coef.pdf}\hfill
\includegraphics[width=0.33\linewidth]{workshop_submission/images/ablation_foreground_thresh.pdf}
\caption{\textbf{Ablation studies on CUB-200-2011.} (Left) Contrastive loss coefficient $\lambda_c$: moderate values achieve best Coverage. (Middle) Foreground loss coefficient $\lambda_{fg}$ (at $\tau_{bg}=0.3$): accuracy and Coverage improve with stronger guidance. (Right) Foreground threshold $\tau_{bg}$ (at $\lambda_{fg}=20$): moderate thresholds improve both accuracy and Coverage.}
\label{fig:ablation_studies}
\end{figure*}

\begin{table}[t]
\centering
\caption{Performance on CUB-200-2011 (DenseNet161).}
\label{tab:main_cub}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{Accuracy} & \textbf{Coverage} & \textbf{Diversity} \\
& (\%) & $\uparrow$ & $\uparrow$ \\
\midrule
ProtoPNet & 76.13 & 0.443 & 0.152 \\
ProtoPShare & 74.40 & 0.594 & 0.184 \\
PixPNet & 76.68 & 0.250 & \textbf{0.450} \\
\midrule
DAPL ($D_1$=32) & 80.96 & 0.514 & 0.221 \\
DAPL ($D_1$=16) & 81.57 & 0.589 & 0.277 \\
DAPL ($D_1$=8) & 80.20 & 0.580 & 0.302 \\
\midrule
DAPL ($D_1$=16) + FG & \textbf{81.69} & \textbf{0.596} & 0.427 \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth, trim={5.5cm 5cm 14cm 6cm}, clip]{workshop_submission/images/cub_head_dim_16.pdf}
\caption{\textbf{Prototype activation comparison.} ProtoPNet (left) shows severe redundancy with 5 background and 2 wing prototypes. DAPL (right) achieves diverse coverage across 10 distinct anatomical parts. Class: American Goldfinch.}
\label{fig:cub_comparison}
\end{figure}

Table~\ref{tab:main_cub} shows DAPL achieves \textbf{81.57\% accuracy} with \textbf{0.589 Coverage}. While PixPNet achieves highest Diversity (0.450) through pixel-level grounding, it suffers from poor Coverage (0.250). ProtoPShare achieves better Coverage (0.594) but reduced accuracy (74.40\%). DAPL with foreground-aware training achieves the best overall balance: 81.69\% accuracy, 0.596 Coverage, and 0.427 Diversity. The optimal $D_1=16$ balances fine-grained details with sufficient context; smaller dimensions ($D_1=8$) enforce Diversity but lose accuracy, while larger ones ($D_1=32$) reduce Diversity and Coverage.

Figure~\ref{fig:cub_comparison} illustrates the improvement: ProtoPNet exhibits severe redundancy with 5 background prototypes and 3 on identical wing patterns, missing critical features. DAPL achieves balanced coverage across 10 distinct anatomical regions (wing, back, belly, leg, crown, beak, neck, nape, forehead). This diversity stems from multi-head attention providing a natural architectural inductive bias---each head specializes in different spatial relationships---while our one-to-one mapping enforces this at the prototype level. Contrastive regularization further pushes prototypes toward distinct representations.

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth, trim={1.6cm 2cm 1.6cm 4.2cm}, clip]{workshop_submission/images/foreground_comparison.pdf}
\caption{\textbf{Foreground-aware training effect.} \textit{Top:} DAPL prototypes exhibit background bias. \textit{Bottom:} DAPL + FG focuses on meaningful bird parts.}
\label{fig:foreground_global}
\end{figure}

Figure~\ref{fig:foreground_global} shows the effect of foreground-aware training: standard DAPL activations extend diffusely into the background, while foreground training localizes them tightly on specific bird parts, explaining the Coverage improvements in Table~\ref{tab:main_cub}.

\subsection{Ablation Studies}

We analyze key hyperparameters on CUB-200-2011 (Figure~\ref{fig:ablation_studies}). Contrastive coefficient $\lambda_c$ controls the balance between diversity enforcement and classification: moderate values achieve the best Coverage (0.600 at $\lambda_c=0.5$) and accuracy (80.98\%), while very low values provide insufficient diversity and very high values over-constrain the model, suggesting that the architectural constraint should be complemented with moderate---not excessive---explicit regularization.

Foreground coefficient $\lambda_{fg}$ shows that increasing foreground guidance steadily improves both accuracy (from 81.17\% to 81.95\%) and Coverage (from 0.446 to 0.596), confirming that directing prototypes toward object features benefits both classification and interpretability. Performance plateaus around $\lambda_{fg}=10.0$-$15.0$.

Background threshold $\tau_{bg}$ reveals an important insight: some background context is beneficial. Allowing moderate background activation ($\tau_{bg}=0.20$-$0.25$) yields the best accuracy (82.02\%) and Coverage (0.584), as prototypes can capture contextual information at object boundaries. Overly strict thresholds ($\tau_{bg} < 0.10$) hurt performance by excluding valid boundary features.

% \textbf{Limitations:} (1) Quantitative evaluation requires part annotations (assessment only, not training); (2) Foreground training requires masks, which may need generation for new domains.

%%%%%%%%% CONCLUSION
\section{Conclusion}

% We presented DAPL, addressing prototype redundancy through architectural constraints enforcing diversity. By leveraging multi-head self-attention with one-to-one prototype assignment and foreground-aware training, DAPL achieves the best overall balance across accuracy, Coverage, and Diversity among all evaluated methods on CUB-200-2011: 81.69\% accuracy, 0.596 Coverage, and 0.427 Diversity with foreground-aware training. Our evaluation framework provides quantitative metrics for systematic interpretability assessment, demonstrating that architectural inductive biases effectively enforce diversity in learned representations.


We presented DAPL, addressing prototype redundancy through multi-head self-attention with one-to-one prototype assignment and foreground-aware training. DAPL achieves the best overall balance across accuracy (81.69\%), Coverage (0.596), and Diversity (0.427) on CUB-200-2011, demonstrating that architectural inductive biases can effectively enforce diversity in learned prototype representations. Our evaluation framework provides quantitative metrics for systematic interpretability assessment, paving the way for more trustworthy prototype-based models.


\section*{Acknowledgments}
This material is based upon work supported in part by the National Science Foundation under Award No.~2429835 and by the Omidyar Network Foundation. The authors acknowledge Research Computing~\cite{rit-rc} at the Rochester Institute of Technology for providing computational resources and support that have contributed to the research results reported in this publication. 



==> workshop_submission/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}
\usepackage{balance}
